Estimating a Common Period for a Set of Irregularly Sampled Functions with Applications to Periodic Variable Star Data

We consider the estimation of a common period for a set of functions sampled at irregular intervals. The problem arises in astronomy, where the functions represent a star's brightness observed over time through different photometric filters. While current methods can estimate periods accurately provided that the brightness is well--sampled in at least one filter, there are no existing methods that can provide accurate estimates when no brightness function is well--sampled. In this paper we introduce two new methods for period estimation when brightnesses are poorly--sampled in all filters. The first, multiband generalized Lomb-Scargle (MGLS), extends the frequently used Lomb-Scargle method in a way that na\"{i}vely combines information across filters. The second, penalized generalized Lomb-Scargle (PGLS), builds on the first by more intelligently borrowing strength across filters. Specifically, we incorporate constraints on the phases and amplitudes across the different functions using a non--convex penalized likelihood function. We develop a fast algorithm to optimize the penalized likelihood by combining block coordinate descent with the majorization-minimization (MM) principle. We illustrate our methods on synthetic and real astronomy data. Both advance the state-of-the-art in period estimation; however, PGLS significantly outperforms MGLS when all functions are extremely poorly--sampled.

==> figs/cep_experiment_output_gamma_table.tex <==
% latex table generated in R 3.1.1 by xtable 1.7-3 package
% Mon Nov 24 18:08:51 2014
\begin{table}[ht]
\centering
\begin{tabular}{lll}
  \hline
\# obs. & gamma1 & gamma2 \\ 
  \hline
5 & 17031.25 & 33.73046875 \\ 
  10 & 550000 & 43.75 \\ 
  15 & 55000 & 1e-48 \\ 
   \hline
\end{tabular}
\end{table}


==> figs/cep_results_output_results.tex <==
% latex table generated in R 3.1.1 by xtable 1.7-3 package
% Mon Nov 24 18:28:51 2014
\begin{table}[t]
\centering
\caption{Fraction of period estimates within 1\% of truth.\label{tab:cep_tab}} 
\begin{tabular}{rrr}
  \hline
obs. / band & GLS & PGLS \\ 
  \hline
  5 & 0.06 & 0.17 \\ 
   10 & 0.64 & 0.69 \\ 
   15 & 0.82 & 0.82 \\ 
   \hline
\end{tabular}
\end{table}


==> figs/sdss_experiment_output_gamma_table.tex <==
% latex table generated in R 3.1.1 by xtable 1.7-3 package
% Tue Dec  2 14:29:51 2014
\begin{table}[ht]
\centering
\begin{tabular}{lll}
  \hline
\# obs. & gamma1 & gamma2 \\ 
  \hline
5 & 21953.125 & 278.6376953125 \\ 
  10 & 84531.25 & 1140.625 \\ 
  15 & 156250 & 550 \\ 
   \hline
\end{tabular}
\end{table}


==> figs/sim2_results_experiment_output_gamma_table.tex <==
% latex table generated in R 3.1.1 by xtable 1.7-3 package
% Mon Nov 24 20:26:21 2014
\begin{table}[ht]
\centering
\begin{tabular}{lll}
  \hline
\# obs. & gamma1 & gamma2 \\ 
  \hline
5 & 6.0625 & 0.131256103515625 \\ 
  10 & 15.625 & 0.182737350463867 \\ 
  15 & 55 & 0.15625 \\ 
   \hline
\end{tabular}
\end{table}


==> figs/sim2_results_results_output_results.tex <==
% latex table generated in R 3.1.1 by xtable 1.7-3 package
% Mon Nov 24 21:31:46 2014
\begin{table}[t]
\centering
\caption{Fraction of period estimates within 1\% of truth.\label{tab:sim2_results_tab}} 
\begin{tabular}{rrr}
  \hline
obs. / band & GLS & PGLS \\ 
  \hline
  5 & 0.04 & 0.23 \\ 
   10 & 0.41 & 0.77 \\ 
   15 & 0.84 & 0.97 \\ 
   \hline
\end{tabular}
\end{table}


==> figs/test_experiment_output_gamma_table.tex <==
% latex table generated in R 3.1.1 by xtable 1.7-3 package
% Tue Nov 18 09:04:24 2014
\begin{table}[ht]
\centering
\begin{tabular}{lll}
  \hline
\# obs. & gamma1 & gamma2 \\ 
  \hline
5 & 0.1 & 0.00325 \\ 
  10 & 0.1 & 0.01 \\ 
  15 & 1e-48 & 1e-48 \\ 
   \hline
\end{tabular}
\end{table}


==> figs/test_results_output_results.tex <==
% latex table generated in R 3.1.2 by xtable 1.7-3 package
% Fri Nov 14 11:25:50 2014
\begin{table}[ht]
\centering
\begin{tabular}{rrr}
  \hline
obs. / band & GLS & PGLS \\ 
  \hline
  5 & 1.00 & 1.00 \\ 
   10 & 1.00 & 1.00 \\ 
   15 & 1.00 & 1.00 \\ 
   \hline
\end{tabular}
\caption{Fraction of period estimates within 5% of truth.\label{tab:test_tab} 
\end{table}


==> figs/test_results_results_output_results.tex <==
% latex table generated in R 3.1.1 by xtable 1.7-3 package
% Wed Oct 15 17:38:07 2014
\begin{table}[ht]
\centering
\begin{tabular}{rrr}
  \hline
\# epochs & ls & bcd \\ 
  \hline
  5 & 0.00 & 0.20 \\ 
   10 & 0.60 & 0.90 \\ 
   15 & 0.80 & 1.00 \\ 
   \hline
\end{tabular}
\end{table}

